Kaleidoscopes, Waves and the Prepotential

Isomorphic flops are topology-changing transitions connecting two diffeomorphic families of Calabi-Yau threefolds. They correspond to the generators of certain Coxeter groups acting on the moduli space. As a consequence of these symmetries, the prepotential of 4D $\mathcal{N} = 2$ Type IIA compactifications on such varieties must assemble into Coxeter-invariant functions. We construct a database of all Coxeter symmetries from isomorphic flops in K\"ahler-favorable CICYs. The action of the Coxeter group on the K\"ahler moduli space leaves a symmetric bilinear form invariant, which we interpret as a metric and construct its associated Laplace-Beltrami operator. We argue that the Coxeter-invariant functions featured in the prepotential solve the Helmholtz equation with this Laplacian, and that the prepotential can then be resummed into a decomposition in terms of eigenfunctions of the Laplace-Beltrami operator. The convergence rate of the raw orbit sums of worldsheet instanton contributions and the resummed expressions are complementary, with the latter sharply localizing around the first few terms in the interior of the moduli space.

==> data/CICY-Coxeter-Database-counts-summary.tex <==
{1} & finite & \SetCell[c=2]{c}{21} &  & \SetCell[c=2]{c}{45} &  & \SetCell[c=2]{c}{165} &  & \SetCell[c=2]{c}{422} &  & \SetCell[c=2]{c}{486} &  & \SetCell[c=2]{c}{294} &  & \SetCell[c=2]{c}{113} &  & \SetCell[c=2]{c}{36} &  & \SetCell[c=2]{c}{8} &  & \SetCell[c=2]{c}{2} &  & \SetCell[c=2]{c}{1592} &  \\
\SetCell[r=2]{c}{{2}} & finite & --- & \SetCell[r=2]{c}{6} & 28 & \SetCell[r=2]{c}{65} & 46 & \SetCell[r=2]{c}{137} & 98 & \SetCell[r=2]{c}{153} & 66 & \SetCell[r=2]{c}{66} & 29 & \SetCell[r=2]{c}{29} & 19 & \SetCell[r=2]{c}{19} & 4 & \SetCell[r=2]{c}{4} & 2 & \SetCell[r=2]{c}{2} & --- & \SetCell[r=2]{c}{---} & 292 & \SetCell[r=2]{c}{481} \\
 & affine & 6 &  & 37 &  & 91 &  & 55 &  & --- &  & --- &  & --- &  & --- &  & --- &  & --- &  & 189 &  \\
\SetCell[r=2]{c}{{3}} & finite & --- & \SetCell[r=2]{c}{---} & --- & \SetCell[r=2]{c}{16} & 10 & \SetCell[r=2]{c}{35} & 10 & \SetCell[r=2]{c}{10} & 8 & \SetCell[r=2]{c}{8} & 6 & \SetCell[r=2]{c}{6} & --- & \SetCell[r=2]{c}{---} & 1 & \SetCell[r=2]{c}{1} & --- & \SetCell[r=2]{c}{---} & --- & \SetCell[r=2]{c}{---} & 35 & \SetCell[r=2]{c}{76} \\
 & indefinite & --- &  & 16 &  & 25 &  & --- &  & --- &  & --- &  & --- &  & --- &  & --- &  & --- &  & 41 &  \\
\SetCell[r=2]{c}{{4}} & finite & --- & \SetCell[r=2]{c}{---} & --- & \SetCell[r=2]{c}{---} & --- & \SetCell[r=2]{c}{14} & 9 & \SetCell[r=2]{c}{9} & --- & \SetCell[r=2]{c}{---} & 3 & \SetCell[r=2]{c}{3} & --- & \SetCell[r=2]{c}{---} & --- & \SetCell[r=2]{c}{---} & --- & \SetCell[r=2]{c}{---} & --- & \SetCell[r=2]{c}{---} & 12 & \SetCell[r=2]{c}{26} \\
 & indefinite & --- &  & --- &  & 14 &  & --- &  & --- &  & --- &  & --- &  & --- &  & --- &  & --- &  & 14 &  \\
{5} & indefinite & \SetCell[c=2]{c}{---} &  & \SetCell[c=2]{c}{---} &  & \SetCell[c=2]{c}{---} &  & \SetCell[c=2]{c}{7} &  & \SetCell[c=2]{c}{---} &  & \SetCell[c=2]{c}{---} &  & \SetCell[c=2]{c}{---} &  & \SetCell[c=2]{c}{---} &  & \SetCell[c=2]{c}{---} &  & \SetCell[c=2]{c}{---} &  & \SetCell[c=2]{c}{7} &  \\

==> data/CICY-Coxeter-Database-summary-diagrams.tex <==
\dynkins{[Coxeter]A1|[Coxeter]A1} & finite & 243 & --- & 6220, 6972, 7240, 7484, 7578, 7588, 7638, 7648, 7714, 7721, 7734, 7735, 7745, 7780, 7788, 7792, 7795, 7841, 7848, 7851, 7877, 7881 & 5245, 5255, 5304, 5305, 5776, 5795, 5805, 5806, 6172, 6200, 6206, 6224, 6524, 6545, 6546, 6558, 6776, 6778, 6809, 6839, 7034, 7045, 7049, 7059, 7075, 7080, 7205, 7245, 7349, 7373, 7449, 7461, 7476, 7478, 7490, 7492, 7495, 7498, 7505, 7574, 7593, 7628, 7649 & 3901, 4079, 4080, 4203, 4223, 4554, 4726, 4727, 4744, 4746, 4763, 4770, 4824, 4839, 5136, 5138, 5249, 5270, 5271, 5313, 5338, 5340, 5353, 5354, 5356, 5379, 5391, 5420, 5448, 5458, 5683, 5711, 5758, 5775, 5798, 5896, 5904, 5912, 5914, 6077, 6083, 6124, 6168, 6169, 6191, 6211, 6236, 6269, 6279, 6323, 6330, 6332, 6543, 6575, 6714, 6726, 6743, 6758, 6764, 6766, 6770, 6783, 6787, 6789, 6804, 6808, 6813, 6823, 6837, 6849, 6850, 6855, 6856, 6869, 6895, 6909, 6915, 6916, 6920, 6921, 6931, 6946, 7194, 7198, 7225, 7257, 7269, 7289, 7442, 7444, 7508, 7526 & 3223, 3234, 3430, 3432, 3485, 3486, 3937, 3955, 3961, 3968, 4027, 4039, 4041, 4118, 4120, 4156, 4160, 4178, 4194, 4195, 4230, 4231, 4866, 4880, 5112, 5114, 5116, 5225, 5233, 5236, 5238, 5343, 5408, 5454, 5476, 5482, 5518, 5753, 5887, 6067, 6099, 6100, 6101, 6135, 6151, 6253, 6286, 6300, 6301, 6302, 6363, 6364, 6367, 6761, 6904, 6943, 7305, 7308 & 2387, 2424, 2485, 2799, 2813, 2822, 3203, 3766, 3829, 3894, 4265, 4314, 4335, 4922, 5110, 6348, 6358 & 1962, 1985, 1999, 2284, 2803, 2894, 4357 & 955, 1466 & 862, 897 \\

\dynkins{[Coxeter]A2} & finite & 21 & --- & 7450, 7481, 7560, 7579, 7779, 7789 & 7200, 7557, 7582 & 6091, 6209, 6239, 6313, 7474, 7494 & 4605, 4606, 4798, 4799, 5723, 5862 & --- & --- & --- & --- \\

\dynkins{[Coxeter]B2} & finite & 28 & --- & --- & --- & --- & 5528, 5552 & 2375, 2701, 2820, 2821, 2857, 2871, 3224, 3524, 4243, 4274, 4342, 4346 & 1620, 1627, 1689, 1702, 1908, 1910, 1920, 2064, 2322, 2683, 3114, 3622 & 1003, 1312 & --- \\

\begin{dynkinDiagram}[Coxeter,label=false]A{**} \dynkinEdgeLabel{1}{2}{\mathrm{H}} \end{dynkinDiagram} & \text{affine} & 26 & 7644, 7726, 7759, 7761, 7799, 7863 & 6771, 7036, 7208, 7316, 7317, 7452, 7530, 7562, 7566, 7610, 7635, 7676, 7708, 7710, 7711, 7717, 7802, 7831, 7842, 7854 & --- & --- & --- & --- & --- & --- & --- \\

\begin{dynkinDiagram}[Coxeter,label=false]A{**} \dynkinEdgeLabel{1}{2}{\mathrm{P}} \end{dynkinDiagram} & \text{affine} & 163 & --- & 6555, 6827, 6971, 7143, 7235, 7366, 7558, 7581, 7584, 7627, 7645, 7755, 7762, 7763, 7824, 7846, 7880 & 4742, 5606, 5794, 6014, 6219, 6275, 6309, 6325, 6328, 6434, 6529, 6547, 6632, 6634, 6677, 6698, 6797, 6905, 6933, 7043, 7044, 7046, 7048, 7054, 7060, 7068, 7089, 7090, 7104, 7110, 7209, 7210, 7227, 7280, 7292, 7301, 7334, 7355, 7357, 7389, 7394, 7402, 7405, 7453, 7456, 7467, 7471, 7473, 7477, 7482, 7483, 7506, 7516, 7517, 7518, 7519, 7520, 7524, 7548, 7569, 7596, 7598, 7605, 7607, 7639, 7650, 7681, 7682, 7690, 7715, 7722, 7723, 7724, 7733, 7738, 7740, 7744, 7751, 7772, 7784, 7786, 7790, 7793, 7796, 7805, 7829, 7837, 7839, 7849, 7852, 7864 & 4151, 4840, 5047, 5879, 5910, 5911, 6240, 6258, 6294, 6326, 6574, 6582, 6583, 6607, 6736, 6737, 6847, 6852, 6864, 6892, 6893, 6901, 6902, 6918, 6919, 6923, 7012, 7096, 7098, 7195, 7272, 7338, 7374, 7379, 7380, 7383, 7393, 7443, 7511, 7547, 7600, 7625, 7651, 7660, 7686, 7687, 7688, 7705, 7741, 7764, 7770, 7794, 7826, 7828, 7830 & --- & --- & --- & --- & --- \\

\dynkins{[Coxeter]A1|[Coxeter]A1|[Coxeter]A1} & finite & 13 & --- & --- & 7217, 7221, 7248, 7250, 7276, 7285 & 6734, 6735, 6805, 6806, 6899, 6900 & --- & --- & --- & 962 & --- \\

\dynkins{[Coxeter]A1|[Coxeter]A2} & finite & 8 & --- & --- & 5784, 5823, 6527, 6557 & 5284, 5285, 5322, 5323 & --- & --- & --- & --- & --- \\

\dynkins{[Coxeter]A1|[Coxeter]B2} & finite & 14 & --- & --- & --- & --- & 3208, 3513, 3905, 4283, 5111, 5167, 5534, 5535 & 2354, 2359, 2682, 2688, 3828, 4315 & --- & --- & --- \\

\CoxDiagramVPH & indefinite & 10 & --- & 7069, 7464, 7485, 7570, 7585, 7587, 7720, 7730, 7843, 7847 & --- & --- & --- & --- & --- & --- & --- \\

\CoxDiagramVPP & indefinite & 21 & --- & --- & 6814, 6815, 7222, 7223, 7274, 7275, 7445, 7446, 7454, 7455, 7458, 7470, 7493, 7497, 7618, 7629, 7654, 7818, 7820, 7825, 7827 & --- & --- & --- & --- & --- & --- \\

\CoxDiagramTriangleAPP & indefinite & 2 & --- & --- & 7042, 7113 & --- & --- & --- & --- & --- & --- \\

\CoxDiagramTrianglePPH & indefinite & 3 & --- & 7727, 7728, 7870 & --- & --- & --- & --- & --- & --- & --- \\

\CoxDiagramTrianglePPP & indefinite & 5 & --- & 5299, 7580, 7669 & 7859, 7860 & --- & --- & --- & --- & --- & --- \\

\dynkins{[Coxeter]A1|[Coxeter]A1|[Coxeter]A2} & finite & 6 & --- & --- & --- & 6732, 6777, 6802, 6834, 6890, 6896 & --- & --- & --- & --- & --- \\

\dynkins{[Coxeter]A2|[Coxeter]A2} & finite & 3 & --- & --- & --- & 5256, 5301, 5452 & --- & --- & --- & --- & --- \\

\dynkins{[Coxeter]B2|[Coxeter]B2} & finite & 3 & --- & --- & --- & --- & --- & 2317, 2335, 2665 & --- & --- & --- \\

\CoxDiagramStarThreeLegP & indefinite & 7 & --- & --- & 7435, 7462, 7491, 7522, 7719, 7736, 7742 & --- & --- & --- & --- & --- & --- \\

\CoxDiagramPStarATwoEdge & indefinite & 6 & --- & --- & 6784, 6828, 7204, 7218, 7241, 7270 & --- & --- & --- & --- & --- & --- \\

\CoxDiagramKFourAllP & indefinite & 1 & --- & --- & 7862 & --- & --- & --- & --- & --- & --- \\

\CoxDiagramStarFourLegFour & indefinite & 5 & --- & --- & --- & 6715, 6788, 6836, 6927, 6947 & --- & --- & --- & --- & --- \\

\CoxDiagramKFiveAllThree & indefinite & 2 & --- & --- & --- & 7447, 7487 & --- & --- & --- & --- & --- \\

==> titlepage-style.tex <==
\RequirePackage{xparse}
\ExplSyntaxOn

% Storage
\seq_new:N \g__tp_preprint_seq
\seq_new:N \g__tp_author_seq
\seq_new:N \g__tp_affil_seq
\seq_new:N \g__tp_email_seq
\tl_new:N  \g__tp_title_tl
\tl_new:N  \g__tp_abstract_tl
\tl_new:N  \g__tp_pdftitle_tl
\box_new:N \l__tp_email_measure_box
\dim_new:N \l__tp_email_rule_dim

% Public “data” commands
\NewDocumentCommand{\Preprint}{m}{
	\seq_gput_right:Nn \g__tp_preprint_seq {#1}
}
\NewDocumentCommand{\Title}{m}{
	\tl_gset:Nn \g__tp_title_tl {#1}
}
\NewDocumentCommand{\Author}{mm}{
	\seq_gput_right:Nn \g__tp_author_seq { {#1}{#2} }
}
\NewDocumentCommand{\Affiliation}{mm}{
	\seq_gput_right:Nn \g__tp_affil_seq { {#1}{#2} }
}
\NewDocumentCommand{\Email}{m}{
	\seq_gput_right:Nn \g__tp_email_seq {#1}
}
\NewDocumentCommand{\Abstract}{m}{
	\tl_gset:Nn \g__tp_abstract_tl {#1}
}
\NewDocumentCommand{\PDFTitle}{m}{
	\tl_gset:Nn \g__tp_pdftitle_tl {#1}
}

% Helpers: formatting items
\cs_new:Npn \__tp_fmt_author:n #1 {
	\__tp_fmt_author_aux:nn #1
}
\cs_new:Npn \__tp_fmt_author_aux:nn #1#2 {
	#1\textsuperscript{#2}
}

\cs_new:Npn \__tp_fmt_affil:n #1 {
	\__tp_fmt_affil_aux:nn #1
}
\cs_new:Npn \__tp_fmt_affil_aux:nn #1#2 {
	\textsuperscript{#1}\textit{#2}
}

\cs_new:Npn \__tp_fmt_email:n #1 {
	\cs_if_exist:NTF \href { \href{mailto:#1}{#1} } { #1 }
}

\cs_new:Npn \__tp_pdfspace {
    \char_generate:nn {32}{12}
}
\newcommand{\TPMakefntext}[1]{\noindent#1}

% Print author list with commas + “and”
\cs_new_protected:Npn \__tp_print_authors: {
	\int_set:Nn \l_tmpa_int { \seq_count:N \g__tp_author_seq }
	\seq_map_indexed_inline:Nn \g__tp_author_seq {
		\__tp_fmt_author:n {##2}
		\int_compare:nNnTF {##1} = {\l_tmpa_int}
			{ }
			{
				\int_compare:nNnTF {##1} = {\l_tmpa_int - 1}
					{~and~}
					{,~}
			}
	}
}

% Print emails comma-separated
% \cs_new_protected:Npn \__tp_print_emails: {
% 	\int_set:Nn \l_tmpa_int { \seq_count:N \g__tp_email_seq }
% 	\int_compare:nNnTF { \l_tmpa_int } = {0}
% 		{ }
% 		{
% 			Email:\,
% 			\int_step_inline:nn { \l_tmpa_int }{
% 				\__tp_fmt_email:n { \seq_item:Nn \g__tp_email_seq {##1} }
% 				\int_compare:nNnTF {##1} = {\l_tmpa_int} { } {,~}
% 			}
% 		}
% }

\cs_new_protected:Npn \__tp_print_emails: {
	\seq_map_inline:Nn \g__tp_email_seq {
		\noindent
		\kern0.66em
		\__tp_fmt_email:n {##1}%
		\kern0.66em
		\par
	}
}

\cs_new_protected:Npn \__tp_set_email_rule_dim: {
	\dim_zero:N \l__tp_email_rule_dim
	\seq_map_inline:Nn \g__tp_email_seq {
		\hbox_set:Nn \l__tp_email_measure_box {
			\footnotesize
			\kern0.66em
			\__tp_fmt_email:n {##1}%
			\kern0.66em
		}
		\dim_compare:nNnT { \box_wd:N \l__tp_email_measure_box } > { \l__tp_email_rule_dim }{
			\dim_set:Nn \l__tp_email_rule_dim { \box_wd:N \l__tp_email_measure_box }
		}
	}
	\dim_compare:nNnT { \l__tp_email_rule_dim } > { \linewidth }{
		\dim_set:Nn \l__tp_email_rule_dim { \linewidth }
	}
}

% Style layer
\NewDocumentCommand{\MakeTitlePage}{}{
	\begingroup

	\seq_if_empty:NF \g__tp_email_seq {
		\__tp_set_email_rule_dim:
		\renewcommand{\footnoterule}{%
			\kern -3pt
			\hrule width \l__tp_email_rule_dim height 0.4pt
			\kern 2.6pt
		}%
	}
    
	% Preprints
	\begin{flushright}
		\seq_map_inline:Nn \g__tp_preprint_seq { {\ttfamily\normalsize ##1}\par }
	\end{flushright}

	% Title block
	\vspace*{40pt}
	\begin{center}
        {\Large\bfseries \tl_use:N \g__tp_title_tl \par}
		\vspace{11mm}

		\__tp_print_authors:
		\par

		\vspace{11mm}
		\small
		\seq_map_inline:Nn \g__tp_affil_seq { \__tp_fmt_affil:n {##1}\par\vspace{3mm} }
	\end{center}

	% Abstract
	\vspace{7mm}
	\begin{abstract}
		\tl_use:N \g__tp_abstract_tl
	\end{abstract}

	% Emails as an unmarked footnote at the bottom of the title page
    \seq_if_empty:NF \g__tp_email_seq {
    	\begingroup
    		\renewcommand{\thefootnote}{}%
    		\expandafter\let\csname @makefntext\endcsname\TPMakefntext
    		\footnotetext{%
    			\raggedright
    			\setlength{\parindent}{0pt}%
    			\__tp_print_emails:
    		}%
    	\endgroup
    }

	\vfill
	\thispagestyle{empty}
	\clearpage
	\endgroup
}

% Front-matter behavior packaged
\NewDocumentCommand{\MakeFrontMatter}{}{
	\MakeTitlePage
	\pagenumbering{roman}
    \begingroup
        \enlargethispage{2\baselineskip} % Force the TOC to fit the extra line
        \tableofcontents
    \endgroup
	\clearpage
	\pagenumbering{arabic}
	\setcounter{page}{1}
}

% PDF metadata
\cs_new:Npn \__tp_author_name:n #1 {
	\__tp_author_name_aux:nn #1
}
\cs_new:Npn \__tp_author_name_aux:nn #1#2 {
	#1
}

\cs_new_protected:Npn \tp_build_pdfauthor_tl:N #1 {
	\tl_clear:N #1
	\int_set:Nn \l_tmpa_int { \seq_count:N \g__tp_author_seq }

	\seq_map_indexed_inline:Nn \g__tp_author_seq {
		\tl_put_right:Nn #1 { \__tp_author_name:n {##2} }

		\int_compare:nNnTF {##1} = {\l_tmpa_int}
			{ }
			{
				\int_compare:nNnTF {##1} = {\l_tmpa_int - 1}
					{
						\tl_put_right:Nx #1 { \__tp_pdfspace }
						\tl_put_right:Nn #1 {and}
						\tl_put_right:Nx #1 { \__tp_pdfspace }
					}
					{
						\tl_put_right:Nn #1 {,}
						\tl_put_right:Nx #1 { \__tp_pdfspace }
					}
			}
	}
}

\makeatletter
\NewDocumentCommand{\SetupPDFMetadataFromTitleData}{}{
	\AtBeginDocument{%
		\@ifundefined{hypersetup}{%
			\PackageWarning{titlepage}{hyperref not loaded, PDF metadata not set}%
		}{%
			% Tell hyperref how to "sanitize" commands appearing in title/author
			\pdfstringdefDisableCommands{%
				\def\textsuperscript##1{}%
				\def\\{ }%
				\def\newline{ }%
				\def\emph##1{##1}%
				\def\textit##1{##1}%
			}%

			% Build plain author string
			\tp_build_pdfauthor_tl:N \l_tmpa_tl

			% Choose PDF title: prefer \PDFTitle if provided, else fall back to \Title
			\tl_if_blank:nTF { \tl_use:N \g__tp_pdftitle_tl }
				{ \tl_set_eq:NN \l_tmpb_tl \g__tp_title_tl }
				{ \tl_set_eq:NN \l_tmpb_tl \g__tp_pdftitle_tl }

			% Let hyperref do the encoding (this avoids the UTF-16LE/BE problems)
			\hypersetup{%
				unicode=true,%
				pdftitle={\tl_use:N \l_tmpb_tl},%
				pdfauthor={\tl_use:N \l_tmpa_tl}%
			}%
		}%
	}%
}
\makeatother

\ExplSyntaxOff
